Manifold for Machine Learning Assurance

The increasing use of machine-learning (ML) enabled systems in critical tasks fuels the quest for novel verification and validation techniques yet grounded in accepted system assurance principles. In traditional system development, model-based techniques have been widely adopted, where the central premise is that abstract models of the required system provide a sound basis for judging its implementation. We posit an analogous approach for ML systems using an ML technique that extracts from the high-dimensional training data implicitly describing the required system, a low-dimensional underlying structure--a manifold. It is then harnessed for a range of quality assurance tasks such as test adequacy measurement, test input generation, and runtime monitoring of the target ML system. The approach is built on variational autoencoder, an unsupervised method for learning a pair of mutually near-inverse functions between a given high-dimensional dataset and a low-dimensional representation. Preliminary experiments establish that the proposed manifold-based approach, for test adequacy drives diversity in test data, for test generation yields fault-revealing yet realistic test cases, and for runtime monitoring provides an independent means to assess trustability of the target system's output.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> sections/discussion.tex <==
Failed ideas.

\subsection{Quality of synthesized inputs?}

How do we determine realism?


\subsection{Limitation of VAE}

Q: Why didn't we evaluate on larger-scale dataset such as ImageNet?
%
No work---at the time of publishing this paper---had succeeded in designing a VAE that is capable of generating 1,000 different classes of high-resolution images.
%
But VAE is an active research topic, and new discoveries are being made.
%
The novelty of this work lies in the idea of generating new inputs from learned manifold and showing the possibility of practical application.
%
We believe that future enhancements in VAE can make our approach scale to more complex tasks.


\subsection{Failure1: latent classifier}


\subsection{Failure2: Use GAN to determine validity}


\subsection{What are the remaining issues?}

To actually defend ourselves saying there isn't any major issue.

\subsection{How is it different from other test gen approaches?}

==> sections/experiment.tex <==

In the experiment, we evaluate the efficacy of DeepDrill in two use-cases of a typical testing workflow.
%
First, we assess whether our technique can synthesize realistic test cases that reveal faults in the model under test.
%
Next, we assess whether synthesized data can be used to augment the training dataset and improve its performance.
%
For a comparison between the two modes of operation---optimization vs. search and filter---we measure the 
%
\begin{itemize}
    \item \textbf{RQ1}: Can we generate realistic test inputs?
    \item \textbf{RQ2}: Can we generate realistic fault-revealing test cases?
    \item \textbf{RQ3}: Does fitness function help identifying realistic fault-revealing test cases with search-based approach?
    \item \textbf{RQ4}: Can we retrain a better model with synthesized inputs?
\end{itemize}



\subsection{Model under test}

\begin{table}[h]
    \centering
    \caption{Models under test}
    \input{tables/models.tex}
    \label{tbl:models}
\end{table}

The experiments are performed with three different models that are designed for three different image classification tasks.
%
The first task is the popular MNIST hand-written digit classification~\cite{lecun1998mnist}.
%
The second task is fashion item image classification task, trained with Fashion-MNIST dataset~\cite{}.
%
Fashion MNIST is designed to be drop-in replacement for MNIST dataset, having the same image resolution and number of classes.
%
However, it is known to be more difficult than MNIST, with the state-of-the-art validation accuracy of 96.7\% with data augmentation.
%https://github.com/xternalz/WideResNet-pytorch
%
The third one is CIFAR10~\cite{krizhevsky2009learning}, which is a ten-class image classification task with 50,000 training data.
%
Although the size of the images is small, the images are full-colored and complex, yet packed in a rather small 32 by 32 by 3 resolution.
%
The state-of-the-art accuracy without extra training data is 97.92\%~\cite{cai2018proxylessnas}.
%
The fourth task is TaxiNet, which is a model designed by our industry partner as a research prototype for taxiing an aircraft automatically an runways and taxiways.
%
Since the original version of TaxiNet is designed to produce continuous values (a cross-track error from the runway center-line and relative heading deviation from the heading of the runway), we modified the design to produce a categorical output only in terms of the cross-track error---namely: far left, left, center, right, far right.


For the structure of the neural networks, we used some of the most popular (and standard) design techniques such as 2D convolution, max-pooling, batch normalization, and weight regularization.
%
Most of all, we used a dropout layer between the convolutions and fully-connected layer so that we can estimate the models' uncertainty using test-time dropout.
%
The details of each model is described in Table~\ref{tbl:models}.


% TaxiNet data collection
%To avoid the high cost of operating an actual aircraft in the real environment,
%we collected the dataset in the X-Plane 11 simulation environment wherein the
%graphics and the dynamics of the environment and the aircraft are accurately
%modeled.
%
%For a preliminary assessment, we fixed the runway to KMWH-04 and the aircraft
%to be Cessna 208B Grand Caravan, while varying the position and the angle of
%the aircraft together with the weather condition.
%
%We used 80,000 samples for training.

\subsection{Training Conditional Two-stage VAEs}

For the implementation of the Conditional Two-stage VAE, we revised the open-sourced TensorFlow code on GitHub~\cite{twostagevae} implemented by the authors of the Two-Stage VAE paper~\cite{dai2019diagnosing}.
%
For MNIST, Fashion MNIST, and CIFAR10, we used the model architecture inspired by InfoGAN~\cite{chen2016infogan}; for TaxiNet, we used the ResNet~\cite{he2016deep}-style architecture which makes use of residual connections inside the deep convolution layers.

\begin{table}[h]
    \centering
    \caption{Trained VAEs}
    \input{tables/vaes.tex}
    \label{tbl:vaes}
\end{table}

The success of a generative model can be measured by how faithfully it can produce a dataset that is similar to the training dataset, both in terms of the quality and the diversity.
%
Fr\'echet Inception Distance (FID) is a widely adopted measure that is shown to correlate well with human judgements~\cite{heusel2017gans}.
%
It measures the Fr\'echet distance between Gaussians fitted over the feature representations of the two datasets---training data and the generated data---where the feature representation is obtained by running a set of data through the Inception V3 network~\cite{szegedy2015going} and extracting 2048-dimensional feature representation in the pool3 bottleneck layer.
%
We report the two FID scores for each VAE---one for reconstructing the validation dataset and another for generating new dataset.
%
The former score shows how faithfully the model can encode and then decode the validation dataset---the set that it was not trained with---and generate the same dataset that it consumed---ideally, the reconstructed images shall look exactly the same to the original validation dataset when the VAE loss (Equation~\ref{eq:vae}) reached its global optimum.
%
The latter score shows the performance of the decoder alone, or the quality of the images generated by sampling from multivariate unit normal distribution over the latent space.
%
Since our goal is to obtain a good generator, we tuned the VAE hyper-parameters for an optimal sampling FID score; lower score indicates a better quality.


The details of each VAE configuration and its FID score is shown in Table~\ref{tbl:vaes}.
%
The size of the latent dimension is a tunable hyper-parameter.
%
Ideally, a ground-truth latent dimension should produce an optimal VAE, when each dimension is fit to encode a latent feature with no redundancy.
%
This latent-dimension, however, is only hypothetical, and we do not have control over the unsupervised process of learning the manifold.
%
In this work, we set the latent dimension to 64 for all the tasks as suggested by Dai and Wipf~\cite{dai2019diagnosing}, and halved them if the sample FID score stays around the same with the size of 32.
%
Although it was argued in their paper that VAEs are trained to ignore superfluous latent dimensions, we observed that finding a smallest possible latent dimension size that retains the generation quality is a key in obtaining in-distribution inputs with our test generation algorithm.


%https://github.com/daib13/TwoStageVAE


\subsection{Implementation and Experiment Setup}

We implemented our test generator in Python to work easily with TensorFlow models.
%
We used a particle swarm optimization package called {\it pyswarm} at the core of our test generation algorithm.
%
The tool and the experiment is publicly available on Github at \url{https://www.github.com/URL}.


The experiments are performed on Ubuntu 16.04 running on an Intel i5 CPU, 32GB
DDR3 RAM, an SSD, and a single NVIDIA GTX 1080-Ti GPU.

==> sections/related.tex <==

A wide adoption of machine learning (ML) in the real-world applications is posing an unprecedented challenge to software testing due to the unique characteristics of the ML systems.
%
Many ML testing approaches had been suggested in recent years for examining properties such as the (adversarial) robustness~\cite{madry2017towards}, correctness~\cite{}, and fairness~\cite{}.
%
For a comprehensive survey on machine learning testing, see the work by Zhang~\etal~\cite{zhang2019machine}.
%
Per their taxonomy, our work presents a novel test case generation technique---both input and oracle---with the goal of testing empirical correctness.


Since the discovery that image classification deep neural networks are easily fooled~\cite{nguyen2014deep,moosavi2016deepfool}, several attempts had been made to facilitate the testing process by generating test inputs~\cite{pei2017deepxplore,tian2017deeptest,zhang2018deeproad,zhou2018deepbillboard}.
%
Most of the approaches can be summarized as utilizing metamorphic testing~\cite{zhu2019datamorphic} in one way or another, and attempt image-to-image transformations from existing datapoints to synthesize new images.
%
DeepXplore~\cite{pei2017deepxplore} is one of the earliest pioneering work which proposed a white-box differential testing approach for generating new inputs.
%
They synthesized new images by applying constraint-preserving transformations on existing datapoints with the objective of jointly maximizing the neuron coverage and the disagreement among the committee of models under test.
%
Their generated inputs, however, are arguably {\it synthetic}, since the transformations---such as occlusions---are visually noticeable and seem unlikely to appear in the real world.
%
Synthetic test inputs---and any technique for adversarial input generation in the same regard~\cite{}---may be desirable if an adversary is assumed, but if the concern is system's correctness under normal operating condition, unrealistic inputs are merely false alarms, for they violate the environmental assumptions.


DeepTest~\cite{tian2017deeptest}, on the other hand, aimed at generating realistic images.
%
They applied metamorphic testing on autonomous driving application and showed that the domain-specific transformations such as fog, rain, and high contrast, can be used to reveal faults in the model under test.
%
DeepRoad~\cite{zhang2018deeproad} stretched this idea further for synthesizing realistic inputs in a sub-domain of the dataset.
%
They aimed at learning complex domain-specific metamorphic transformations so that new inputs can be synthesized beyond simple computer-vision-based transformations.
%
They used a variant of generative adversarial network (GAN)~\cite{goodfellow2014generative} called UNIT~\cite{liu2017unsupervised} for this transformation, which allowed them to transform sunny road images to to snowy or rainy road images with high visual quality.
%
This approach, however, requires effort in constructing such domain-specific image translators which inevitably involves collecting lots of images from which to learn the desired {\it style}.
%
In comparison, our approach does not require additional data beyond training dataset, yet is able to generate inputs beyond the existing dataset.
%
Moreover, our approach does not rely on metamorphic data transformation, but rather sample the pair of input and oracle from the learned manifold.

{\bf I want to argue: "We believe that our work is complementary to metamorphic approaches." Should I do this here or in the discussion?}


In spirit, the key idea of this work can be summarized as applying search-based testing on the manifold space, which is similar to the idea presented in a positional paper by Yoo~\cite{yoo2019sbst} as a potential possibility.
%
Our work is, in a sense, a substantial concretization of this idea, and answers the question with full-bodied development of the technique.

{\bf Talk about some of the search-based testing works.}

{\bf Talk about some VAE works: "VAE is still an active research topic."}

\begin{comment}
    {\bf Adversarial Examples.}
    Since the discovery of adversarial examples, which are attack vectors which can fool neural networks, 
    %
    Deep neural networks are easily fooled~\cite{nguyen2014deep}.
    %
    DeepFool~\cite{moosavi2016deepfool}.
    %
    Universal adversarial perturbation~\cite{moosavi2017universal} showed that a universal attack vector can be generated for any given neural network under attack which can fool the network with high probability yet with an unnoticeable amount of visual perturbation.
\end{comment}



==> sections/result.tex <==

We ran our manifold-based test generator with the models under test in the loop, for generating fault-revealing test cases tailored for the models under test.
%
This section presents the result and address the two research questions.


\subsection{Can we generate realistic test inputs?}

As introduced earlier in Section~\ref{}, we used Fr\'echet Inception Distance (FID) as a quantitative measure of realism, and presented the scores in Table~\cite{twostagevae}.
%
As the values indicate the degree of discrepancy between the original dataset and the generated one, any non-zero FID score indicates that the generated inputs are different to the original dataset to some extent, and possibly unreal.
%
However, we observed that the score alone cannot be used as an objective measure to determine the realism.
%
For instance, a dataset with a higher FID score may {\it look more real} than another dataset with a lower score.
%
As a complementary qualitative measure of visual quality, we present the original and the reconstructed images side by side in Figure~\ref{fig:reconstruction}.
%
The reconstruction quality serves as a sanity check of trained VAEs---if the pair of encoder and decoder is well trained, it should at least be able to reconstruct the original validation dataset well.
%
{\bf TODO: keep on writing.}

\begin{figure*}[t]
    \subfloat[MNIST]{
        \includegraphics[width=0.18\textwidth]{figures/mnist_original.png}
        \label{fig:mnist_original}
    }
    \subfloat[Fashion MNIST]{
        \includegraphics[width=0.18\textwidth]{figures/fashion_original.png}
        \label{fig:fashion_original}
    }
    \subfloat[CIFAR10]{
        \includegraphics[width=0.18\textwidth]{figures/cifar_original.png}
        \label{fig:cifar_original}
    }
    \subfloat[TaxiNet]{
        \includegraphics[width=0.34\textwidth]{figures/taxinet_original.png}
        \label{fig:taxinet_original}
    }
    
    \subfloat[MNIST]{
        \includegraphics[width=0.18\textwidth]{figures/mnist_recon.png}
        \label{fig:mnist_original}
    }
    \subfloat[Fashion MNIST]{
        \includegraphics[width=0.18\textwidth]{figures/fashion_recon.png}
        \label{fig:fashion_original}
    }
    \subfloat[CIFAR10]{
        \includegraphics[width=0.18\textwidth]{figures/cifar_recon.png}
        \label{fig:cifar_original}
    }
    \subfloat[TaxiNet]{
        \includegraphics[width=0.34\textwidth]{figures/taxinet_recon.png}
        \label{fig:taxinet_original}
    }
    \caption{Images reconstructed by trained VAE (original images in the upper row; reconstructed images in the lower row). The reconstructed images look realistic overall, although some fine-grained texture is lost for Fashion MNIST and TaxiNet. CIFAR10 images, however, are too blurry that the objects are not recongnizable.}
    \label{fig:reconstruction}
\end{figure*}

\begin{figure*}
    %\centering
    %\hfill
    \subfloat[MNIST]{
        \includegraphics[width=0.25\textwidth]{figures/mnist_sample.png}
        \label{fig:mnist_samples}
    }
    %\centering
    %\hfill
    \subfloat[Fashion MNIST]{
        \includegraphics[width=0.25\textwidth]{figures/fashion_sample.png}
        \label{fig:fashion_samples}
    }
    \subfloat[TaxiNet]{
        \includegraphics[width=0.45\textwidth]{figures/taxint_sample.png}
        \label{fig:taxinet_samples}
    }
    \caption{
    Images generated by the Two-stage VAEs, sampled from the second-stage latent space per each class (no cherry-picking). Diverse range of realistic images are generated. }
    \label{fig:vae_samples}
\end{figure*}

The visual quality of the images generated by the trained VAEs is shown in Figure~\ref{fig:vae_samples}.
%
Each row of images are generated with the same class conditioning. From the top to the bottom, MNIST classes range from 0 to 9; Fashion MNIST classes are t-shirt/top, trouser, pullover, dress, coat, sandal, shirt, sneaker, bag, ankle boot; TaxiNet classes are far right, right, center, left, far left.
%
We can see that most of the images are very crisp and almost indistinguishable from the original images.
%
Each image matches the label it was conditioned with, and different varieties appear within the same class.

\subsection{Can we generate fault-revealing test cases?}

For each model under test, we attempted generating a thousand test cases.
%
We call it an {\it attempt} because not all the generated inputs may be valid in terms of the real input distribution.
%
As there is a tension---and trade-off---between the two optimization terms in Equation~\ref{eq:opt}, or between the realism of the inputs and its fault-revealing, some inputs may be sampled from out of the distribution.
%
These out-of-distribution cases cannot be filtered out automatically because the real data distribution is beyond a logical specification.
%
We used human as oracle to determine whether each test case---or a pair of image and label---is valid or not.
%
We argue that this yes-or-no question is a much simpler task than labeling the image from the scratch, especially as the number of classes increases.

\begin{figure*}[h]
    \centering
    \subfloat[MNIST]{
        \includegraphics[width=0.3\textwidth]{figures/digits.png}
        \label{fig:faults_mnist}
    }
    \caption{Fault-revealing test cases (cherry-picked)}
    \label{fig:faults}
\end{figure*}

Figure~\ref{fig:mnist_result} showcases some of the fault-revealing test cases after filtering out invalid ones.
%

\begin{table*}[]
    \centering
    \caption{Generated test cases}
    \label{tab:result}
    \input{tables/result.tex}
\end{table*}


\subsection{Can generated inputs help understand the models' weakness?}

{\bf Move it to the discussion. Confusion matrix, latent variable mapping, faulty region focused drilling.}

\subsection{Threats to Validity}

Determining the validity of images is inevitably a subjective judgement.
%
We ensured that an objective decision is made by having two people making judgements, and the same set of people apply the same set of criteria in marking invalid images.

The experiment was performed with only one particular kind of search metaheuristic.
%
The result may be different if different search algorithm was applied.


==> tables/models.tex <==
\small
\begin{tabular}{@{}lllllll@{}}
\toprule
Task    & \begin{tabular}[c]{@{}l@{}}Image\\ Resolution\end{tabular} & \begin{tabular}[c]{@{}l@{}}\# Train\\ data\end{tabular} & \begin{tabular}[c]{@{}l@{}}\# Val.\\ data\end{tabular} & \begin{tabular}[c]{@{}l@{}}Train\\ acc.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Val\\ acc.\end{tabular} & \begin{tabular}[c]{@{}l@{}}\# Train\\ params\end{tabular} \\ \midrule
MNIST   & $28 \times 28 \times 1$                                    & 60,000                                                  & 10,000                                                 & 99.38\%                                              & 99.15\%                                            & 594,922                                                   \\
Fashion & $28 \times 28 \times 1$                                    & 60,000                                                  & 10,000                                                 & 99.86\%                                              & 92.71\%                                            & 858,026                                                   \\
TaxiNet & $100 \times 180 \times 3$                                  & 80,000                                                  & 20,000                                                 &                                                      &                                                    &                                                           \\ \bottomrule
\end{tabular}

==> tables/result.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}
\centering
\small
\begin{tabular}{lrrrrrrrrrrr} 
\toprule
        & \multicolumn{5}{c}{Optimization} & \multicolumn{5}{c}{Sampling}                                                                                                                    & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}labeling\\cost \end{tabular}}}  \\ 
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
        & \multicolumn{1}{l}{Generated} & \multicolumn{1}{l}{Time} & \multicolumn{1}{c}{FF. Count} & \multicolumn{1}{c}{Valid} & \multicolumn{1}{c}{FID} & \multicolumn{1}{l}{Generated} & \multicolumn{1}{l}{Time} & \multicolumn{1}{c}{FF. Count} & \multicolumn{1}{c}{Valid} & \multicolumn{1}{c}{FID} & \multicolumn{1}{c}{}                                                                          \\ 
\midrule
MNIST   & 3,222                         & 30m25s                   & 1000                          & ?                         & ?                       & 300,256                       & 5m 42s                   & 1000                          & 663                       & 29.36 \$pm\$ 0.06       & 1.7s/ea.                                                                                      \\
Fashion &                               &                          & 1000                          &                           &                         & 12,128                        & 6m 57s                   & 1000                          & 687                       & 69.74 \$pm\$ 0.19       & 2.0s/ea.                                                                                      \\
TaxiNet & 11,073                        & 10h 13m                  & 1000                          &                           &                         &                               &                          &                               &                           &                         & 2.3s/ea.                                                                                      \\
\bottomrule
\end{tabular}

==> tables/vaes.tex <==
\small
\begin{tabular}{@{}lrrrrr@{}}
\toprule
        & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Trainable\\ parameters\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Training\\ time\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Latent\\ dimension\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}FID\\ recon.\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}FID\\ sample\end{tabular}} \\ \midrule
MNIST   & 21,860,515 & 5h 21m & 32 & 6.64 & 8.80 \\
Fashion & 21,860,515 & 8h 19m & 32 & 17.97 & 23.86 \\
CIFAR10 & 26,074,053 & 6h 19m & 64 & 78.06 & 91.49 \\
TaxiNet & 41,294,597 & 13h 42m & 32 & 161.32 & 157.65 \\ \bottomrule
\end{tabular}
